Efficient Audio Captioning with Encoder-Level Knowledge Distillation

Significant improvement has been achieved in automated audio captioning (AAC) with recent models. However, these models have become increasingly large as their performance is enhanced. In this work, we propose a knowledge distillation (KD) framework for AAC. Our analysis shows that in the encoder-decoder based AAC models, it is more effective to distill knowledge into the encoder as compared with the decoder. To this end, we incorporate encoder-level KD loss into training, in addition to the standard supervised loss and sequence-level KD loss. We investigate two encoder-level KD methods, based on mean squared error (MSE) loss and contrastive loss, respectively. Experimental results demonstrate that contrastive KD is more robust than MSE KD, exhibiting superior performance in data-scarce situations. By leveraging audio-only data into training in the KD framework, our student model achieves competitive performance, with an inference speed that is 19 times faster\footnote{An online demo is available at \url{https://huggingface.co/spaces/wsntxxn/efficient_audio_captioning}}.

==> rebuttal.tex <==
Thanks for the careful review and insightful comments from all reviewers.
Review 1 said a detailed analysis of how each type of loss contribute individually. In fact, we conducted such analysis and the result demonstrated that each loss improves the final result and the sequence-level KD loss contributes the most. However, since the space is rather limited, we do not include it in the manuscript. Instead, we perform the inference speedup test because it is more related to practical application of audio captioning models.
Besides, review 1 suggests that there is a need for improvement in the readability of the tables.
We will split the table into three parts: 1) previous methods; 2) the teacher model; 3) the distilled student with different configurations, to make the result clearer.

